Breaking through Deterministic Barriers: Randomized Pruning Mask Generation and Selection

It is widely acknowledged that large and sparse models have higher accuracy than small and dense models under the same model size constraints. This motivates us to train a large model and then remove its redundant neurons or weights by pruning. Most existing works pruned the networks in a deterministic way, the performance of which solely depends on a single pruning criterion and thus lacks variety. Instead, in this paper, we propose a model pruning strategy that first generates several pruning masks in a designed random way. Subsequently, along with an effective mask-selection rule, the optimal mask is chosen from the pool of mask candidates. To further enhance efficiency, we introduce an early mask evaluation strategy, mitigating the overhead associated with training multiple masks. Our extensive experiments demonstrate that this approach achieves state-of-the-art performance across eight datasets from GLUE, particularly excelling at high levels of sparsity.

==> figs/abl4.tex <==
\begin{figure}[!htb]
    \centering
    \subfigure[MRPC]{
        \includegraphics[trim= 0 10 0 40, clip, width=0.22\textwidth]{imgs/mrpc_vs_mnli_1.png}
        \label{abl4:a}
    }
    \subfigure[MNLI-m]{
        \includegraphics[trim= 0 10 0 40, clip, width=0.22\textwidth]{imgs/mrpc_vs_mnli_2.png}
        \label{abl4:b}
    }
    \caption{Impact of different dataset size: MRPC (\ref{abl4:a}) and MNLI-M(\ref{abl4:b}). The value on the vertical axis indicates model accuracy. The value on the horizontal axis represents the amount of introduced robustness}
    \label{abl:4}
\end{figure}

==> src/8-acknowledgement.tex <==
\section*{Acknowledgements}

This paper is supported by Moffett AI Research.

==> src/rebuttal.tex <==
Certainly! Let's delve deeper into the potential pitfalls by providing more detailed examples:

- **Neural Network Output Equation:**
      \[ Y = w_i \cdot F_i \]
  
    **Explanation:**
    - \( Y \) denotes the network output.
    - \( F_i \) signifies a specific feature.
    - \( w_i \) is the weight associated with that feature.
    
   **Magnitude-based Pruning Process:**   
    - Prune the term \( w_i \cdot F_i \) if \( |w_i| < T \).

   **Potential Pitfall of Magnitude-based Pruning with Examples:**  
    - The effect of a feature on \( Y \) is not exclusively determined by the magnitude of \( w_i \). It's a compounded result of both \( w_i \) and the sensitivity or importance of \( F_i \).
        - **High sensitivity (Example)**: Suppose \( F_i \) represents the sharpness of an image, a small change in sharpness (even if \( w_i \) is small) might drastically affect our recognition of an object in the image. Thus, even if \( |w_i| = 0.01 \) (small weight), the influence of \( F_i \) could make a difference of 0.5 in \( Y \), making it critical.
        - **Low sensitivity (Example)**: On the other hand, consider \( F_i \) representing the hue of the image background. Even if this hue has a large weight \( w_i = 5 \), a change in the background hue might not alter our recognition much, making the product \( w_i \cdot F_i \) yield only a minimal difference of 0.1 in \( Y \).
  
   **Key Takeaway:**  
    - The decision to remove weights based on their influence on \( Y \) should consider more than just the weight \( w_i \). It should also account for the sensitivity of the feature \( F_i \). By not doing so, we risk discarding features with small weights that might have high sensitivities and profound impacts on \( Y \). The strict magnitude-based approach can introduce a "lack of variety," potentially missing this nuanced relationship.
